Application-Driven Exascale: The JUPITER Benchmark Suite

Benchmarks are essential in the design of modern HPC installations, as they define key aspects of system components. Beyond synthetic workloads, it is crucial to include real applications that represent user requirements into benchmark suites, to guarantee high usability and widespread adoption of a new system. Given the significant investments in leadership-class supercomputers of the exascale era, this is even more important and necessitates alignment with a vision of Open Science and reproducibility. In this work, we present the JUPITER Benchmark Suite, which incorporates 16 applications from various domains. It was designed for and used in the procurement of JUPITER, the first European exascale supercomputer. We identify requirements and challenges and outline the project and software infrastructure setup. We provide descriptions and scalability studies of selected applications and a set of key takeaways. The JUPITER Benchmark Suite is released as open source software with this work at https://github.com/FZJ-JSC/jubench.

==> author-blind.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}


==> makefile <==
# --------------------------------------------------------------------------------------------------
# SPDX-License-Identifier: Apache-2.0
# Copyright (C) 2021-2021, Jayesh Badwaik <jayesh@badwaik.dev>
# --------------------------------------------------------------------------------------------------
include document.mk
TEMPORARY_DIR=tmp
RELEASE_BUILD_DIR=${TEMPORARY_DIR}/release
DEBUG_BUILD_DIR=${TEMPORARY_DIR}/debug
VERBOSE_BUILD_DIR=${TEMPORARY_DIR}/verbose


ifndef VERBOSE
.SILENT:
endif

release:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -lualatex -interaction=nonstopmode \
		-logfilewarnings- -quiet \
		-outdir=${RELEASE_BUILD_DIR} -gg -cd \
		-auxdir=${RELEASE_BUILD_DIR} \
		${MAINFILE}.tex &> /dev/null
	cp ${RELEASE_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."

debug:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -lualatex -interaction=nonstopmode \
		-logfilewarnings- -quiet -shell-escape \
		-outdir=${DEBUG_BUILD_DIR} -gg -cd \
		-auxdir=${DEBUG_BUILD_DIR} \
		${MAINFILE}.tex
	cp ${DEBUG_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."

verbose:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -lualatex -interaction=nonstopmode \
		-logfilewarnings- -shell-escape -verbose \
		-outdir=${VERBOSE_BUILD_DIR} -gg -cd \
		-auxdir=${VERBOSE_BUILD_DIR} \
		${MAINFILE}.tex
	cp ${VERBOSE_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."


clean:
	rm ${MAINFILE}.pdf



==> setup.tex <==
\usepackage{fancyhdr}
\usepackage[T1]{fontenc}
\IEEEoverridecommandlockouts
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage[svgnames]{xcolor}
\usepackage{academicons}
\usepackage{hyperref}
\usepackage{siunitx}
\RequirePackage{csquotes}
\RequirePackage[
backend=biber,
giveninits=true,
style=ieee
]
{biblatex}

\usepackage{booktabs}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}
\usepackage{comment}

\usepackage{orcidlink}
\usepackage[hyperfirst=false]{glossaries-prefix}
\glsdisablehyper
\usepackage[flushleft]{threeparttable}
\usepackage{dblfloatfix}

\usepackage{tabularray}
\UseTblrLibrary{booktabs}

\newcommand{\myrot}[1]{\rlap{\rotatebox{90}{#1}}}
\newcommand*\circled[1]{\tikz[baseline=(char.base),overlay]{\node[shape=circle,fill=gray,text=white,font=\scriptsize,inner sep=2pt] (char) {#1};}}

\definecolor{fzjblue}{RGB}{2,61,107}
\definecolor{fzjlightblue}{RGB}{173,189,227}
\definecolor{fzjgray}{RGB}{235,235,235}
\colorlet{fzjgrey}{fzjgray}
\definecolor{fzjred}{RGB}{235, 95, 115}
\definecolor{fzjgreen}{RGB}{185, 210, 95}
\definecolor{fzjyellow}{RGB}{250, 235, 90}
\definecolor{fzjviolet}{RGB}{175, 130, 185}
\definecolor{fzjorange}{RGB}{250, 180, 90}
\definecolor{fzjblack}{RGB}{0,0,0}
\definecolor{fzjwhite}{RGB}{255,255,255}

\sisetup{                                                   
    per-mode=symbol,
    separate-uncertainty,
    list-units=repeat,
    range-units=repeat,
}
\DeclareSIUnit\flop{\textsc{Fl}\textsc{Op}}
\DeclareSIUnit\cycle{\textsc{Cycle}}
\DeclareSIUnit[per-mode=symbol]\floppersec{\flop\per\second}
\DeclareSIUnit[per-mode=symbol]\flopperjoule{\flop\per\joule}
\DeclareSIQualifier{\doubleprecision}{FP64}
\DeclareSIQualifier{\singleprecision}{FP32}
\DeclareSIQualifier{\halfprecision}{FP16}
\DeclareSIQualifier{\theoretical}{th}
\DeclareSIUnit\pixel{px}
\newcommand{\doubleblind}[1]{}  %

